Detect, Augment, Compose, and Adapt: Four Steps for Unsupervised Domain Adaptation in Object Detection

Unsupervised domain adaptation (UDA) plays a crucial role in object detection when adapting a source-trained detector to a target domain without annotated data. In this paper, we propose a novel and effective four-step UDA approach that leverages self-supervision and trains source and target data concurrently. We harness self-supervised learning to mitigate the lack of ground truth in the target domain. Our method consists of the following steps: (1) identify the region with the highest-confidence set of detections in each target image, which serve as our pseudo-labels; (2) crop the identified region and generate a collection of its augmented versions; (3) combine these latter into a composite image; (4) adapt the network to the target domain using the composed image. Through extensive experiments under cross-camera, cross-weather, and synthetic-to-real scenarios, our approach achieves state-of-the-art performance, improving upon the nearest competitor by more than 2% in terms of mean Average Precision (mAP). The code is available at https://github.com/MohamedTEV/DACA.

==> images/mixing_schemes.tex <==
\begin{figure}[t]
    \centering
    \subfigure[Source \cite{sim10k}]{\includegraphics[width=0.19\textwidth]{images/src.jpg}} 
    \subfigure[Target \cite{cityscapes}]{\includegraphics[width=0.19\textwidth]{images/trg.jpg}} 
    \subfigure[CutMix \cite{cutmix}]{\includegraphics[width=0.19\textwidth]{images/cutmix.jpg}} 
    \subfigure[ConfMix \cite{confmix}]{\includegraphics[width=0.19\textwidth]{images/confmix.jpg}}
    \subfigure[\ourmethod]{\includegraphics[width=0.19\textwidth]{images/TransMix.jpg}}
    \bigskip
    \vspace{-3mm}
    \caption{
    Comparison between \ourmethod and competitor mixing schemes.
    Green bounding boxes are ground-truth annotations, red bounding boxes are pseudo-detections.
    Unlike \ourmethod, both CutMix~\cite{cutmix} and ConfMix~\cite{confmix} require source images to compose the mixed image.
    }
    \label{fig:mixingschemes}
\end{figure}

==> images/teaser/teaser1.tex <==
\begin{figure}
\centering

\begin{tikzpicture}

%
% First row
%

\node [anchor=south west, inner sep=0] at (0.0,0.0) {\includegraphics[width=22mm]{images/teaser/src}};
% \fill [white, opacity=0.75] (0.0,0.0) rectangle (1.1,0.61); % bottom left
% \fill [white, opacity=0.75] (0.0,0.61) rectangle (1.1,1.22); % top left
% \fill [white, opacity=0.75] (1.1,0.0) rectangle (2.22,0.61); % bottom right
\fill [white, opacity=0.75] (1.1,0.61) rectangle (2.22,1.22); % top right
\draw [white, dashed, line width=0.75] (0.0,0.61) -- (2.22,0.61) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (1.1,0.0) -- (1.1,1.22) {};
\draw [black, line width=0.75] (0.0,0.0) rectangle (2.2,1.22) {};
\node at (1.1,-0.3) {\small $\textbf{X}_S$};

% \node [anchor=south west, inner sep=0] at (2.4,0.0) {\includegraphics[width=22mm]{images/teaser/trg}};
% \fill [white, opacity=0.75] (2.4,0.0) rectangle (3.5,0.61); % bottom left
% \fill [white, opacity=0.75] (2.4,0.61) rectangle (3.5,1.22); % top left
% \fill [white, opacity=0.75] (3.5,0.0) rectangle (4.62,0.61); % bottom right
% \draw [white, dashed, line width=0.75, opacity=0.75] (2.4,0.61) -- (4.62,0.61) {};
% \draw [white, dashed, line width=0.75, opacity=0.75] (3.5,0.0) -- (3.5,1.22) {};
% \draw [black, line width=0.75] (2.4,0.0) rectangle (4.6,1.22) {};
% \node at (3.5,-0.3) {\small $\textbf{X}_T$};

\node [anchor=south west, inner sep=0] at (3.8,0.0) {\includegraphics[width=22mm]{images/teaser/src}};
\node [anchor=south west, inner sep=0] at (4.9,0.605) {\includegraphics[width=11mm]{images/teaser/trg_crop}};
\draw [white, dashed, line width=0.75, opacity=0.75] (3.8,0.61) -- (6.02,0.61) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (4.9,0.0) -- (4.9,1.22) {};
\draw [black, line width=0.75] (3.8,0.0) rectangle (6.0,1.22) {};
\node at (4.9,-0.3) {\small $\hat{\textbf{X}}_T = \frac{3}{4}\textbf{X}_S + \frac{1}{4}\textbf{X}_T$};

\fill [orange, opacity=0.75] (6.2,0.01) rectangle (8.4,1.219) {};
\fill [white, opacity=0.75] (7.3,0.61) rectangle (8.42,1.22) {};
\draw [white, dashed, line width=0.75] (6.2,0.61) -- (8.42,0.61) {};
\draw [white, dashed, line width=0.75] (7.3,0.0) -- (7.3,1.22) {};
\draw [black, line width=0.75] (6.2,0.0) rectangle (8.4,1.22) {};
\node at (7.3,-0.25) {\small Redundant info.};

%
% Second row
%

\node [anchor=south west, inner sep=0] at (0.0,-2.0) {\includegraphics[width=22mm]{images/teaser/trg}};
\fill [white, opacity=0.75] (0.0,-2.0) rectangle (1.1,-1.39); % bottom left
\fill [white, opacity=0.75] (0.0,-1.39) rectangle (1.1,-0.78); % top left
\fill [white, opacity=0.75] (1.1,-2.0) rectangle (2.22,-1.39); % bottom right
\draw [white, dashed, line width=0.75, opacity=0.75] (0.0,-1.39) -- (2.22,-1.39) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (1.1,-2.0) -- (1.1,-0.78) {};
\draw [black, line width=0.75] (0.0,-2.0) rectangle (2.2,-0.78) {};
\node at (1.1,-2.3) {\small $\textbf{X}_T$};

\node [anchor=south west, inner sep=0] at (3.8,-1.395) {\includegraphics[width=11mm]{images/teaser/aug2}}; % top left
\node [anchor=south west, inner sep=0] at (4.9,-1.395) {\includegraphics[width=11mm]{images/teaser/aug1}}; % top right
\node [anchor=south west, inner sep=0] at (3.8,-2.0) {\includegraphics[width=11mm]{images/teaser/aug4}}; % bottom left
\node [anchor=south west, inner sep=0] at (4.9,-2.0) {\includegraphics[width=11mm]{images/teaser/aug3}}; % bottom right
\draw [white, dashed, line width=0.75, opacity=0.75] (3.8,-1.39) -- (6.02,-1.39) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (4.9,-2.0) -- (4.9,-0.78) {};
\draw [black, line width=0.75] (3.8,-2.0) rectangle (6.0,-0.78) {};
\node at (4.9,-2.3) {\small $\hat{\textbf{X}}_T$};

\fill [orange, opacity=0.25] (6.2,-2.0) rectangle (8.42,-0.78) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (6.2,-1.39) -- (8.42,-1.39) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (7.3,-2.0) -- (7.3,-0.78) {};
\draw [black, line width=0.75] (6.2,-2.0) rectangle (8.42,-0.78) {};
\node at (7.3,-2.25) {\small Redundant info.};

%
% Arrows
%

\fill [fill=blue!75, opacity=0.75] (2.3,1.22) -- (3.7,0.61) -- (2.3,0.61);
\fill [fill=blue!75, opacity=0.75] (2.3,0.61) -- (3.7,0.61) -- (2.3,-2.0);
\node at (2.9,0.56) {\small \color{white}{ ConfMix}};

\fill [fill=red!75, opacity=0.75] (2.5,-2.0) -- (3.7,-1.39) -- (2.5,-1.39);
\fill [fill=red!75, opacity=0.75] (2.5,-1.39) -- (3.7,-1.39) -- (2.5,-0.78);
\node at (2.97,-1.362) {\small \color{white}{ \ourmethod}};

\end{tikzpicture}

\vspace{2mm}
\caption{
\davidecomment{Mohamed, please add the caption.}
}
\mohamedcomment{Sure, when the teaser is done i will inspire from it.}
}
\label{fig:teaser}

\end{figure}

==> images/teaser/teaser2.tex <==
\begin{figure}
\centering

\floatbox[{\capbeside\thisfloatsetup{capbesideposition={right,top},capbesidewidth=4cm}}]{figure}[\FBwidth]
{\caption{TOTO}\label{fig:teaser}}
{
\begin{tikzpicture}

%
% First row
%

\node [anchor=south west, inner sep=0] at (0.0,0.0) {\includegraphics[width=22mm]{images/teaser/src}};
% \fill [white, opacity=0.75] (0.0,0.0) rectangle (1.1,0.61); % bottom left
% \fill [white, opacity=0.75] (0.0,0.61) rectangle (1.1,1.22); % top left
% \fill [white, opacity=0.75] (1.1,0.0) rectangle (2.22,0.61); % bottom right
\fill [white, opacity=0.75] (1.1,0.61) rectangle (2.22,1.22); % top right
\draw [white, dashed, line width=0.75] (0.0,0.61) -- (2.22,0.61) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (1.1,0.0) -- (1.1,1.22) {};
\draw [black, line width=0.75] (0.0,0.0) rectangle (2.2,1.22) {};
\node at (1.1,-0.3) {\small $\textbf{X}_S$};

% \node [anchor=south west, inner sep=0] at (2.4,0.0) {\includegraphics[width=22mm]{images/teaser/trg}};
% \fill [white, opacity=0.75] (2.4,0.0) rectangle (3.5,0.61); % bottom left
% \fill [white, opacity=0.75] (2.4,0.61) rectangle (3.5,1.22); % top left
% \fill [white, opacity=0.75] (3.5,0.0) rectangle (4.62,0.61); % bottom right
% \draw [white, dashed, line width=0.75, opacity=0.75] (2.4,0.61) -- (4.62,0.61) {};
% \draw [white, dashed, line width=0.75, opacity=0.75] (3.5,0.0) -- (3.5,1.22) {};
% \draw [black, line width=0.75] (2.4,0.0) rectangle (4.6,1.22) {};
% \node at (3.5,-0.3) {\small $\textbf{X}_T$};

\node [anchor=south west, inner sep=0] at (3.8,0.0) {\includegraphics[width=22mm]{images/teaser/src}};
\node [anchor=south west, inner sep=0] at (4.9,0.605) {\includegraphics[width=11mm]{images/teaser/trg_crop}};
\draw [white, dashed, line width=0.75, opacity=0.75] (3.8,0.61) -- (6.02,0.61) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (4.9,0.0) -- (4.9,1.22) {};
\draw [black, line width=0.75] (3.8,0.0) rectangle (6.0,1.22) {};
\node at (4.9,-0.3) {\small $\hat{\textbf{X}}_T = \frac{3}{4}\textbf{X}_S + \frac{1}{4}\textbf{X}_T$};

%
% Second row
%

\node [anchor=south west, inner sep=0] at (0.0,-2.0) {\includegraphics[width=22mm]{images/teaser/trg}};
\fill [white, opacity=0.75] (0.0,-2.0) rectangle (1.1,-1.39); % bottom left
\fill [white, opacity=0.75] (0.0,-1.39) rectangle (1.1,-0.78); % top left
\fill [white, opacity=0.75] (1.1,-2.0) rectangle (2.22,-1.39); % bottom right
\draw [white, dashed, line width=0.75, opacity=0.75] (0.0,-1.39) -- (2.22,-1.39) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (1.1,-2.0) -- (1.1,-0.78) {};
\draw [black, line width=0.75] (0.0,-2.0) rectangle (2.2,-0.78) {};
\node at (1.1,-2.3) {\small $\textbf{X}_T$};

\node [anchor=south west, inner sep=0] at (3.8,-1.395) {\includegraphics[width=11mm]{images/teaser/aug2}}; % top left
\node [anchor=south west, inner sep=0] at (4.9,-1.395) {\includegraphics[width=11mm]{images/teaser/aug1}}; % top right
\node [anchor=south west, inner sep=0] at (3.8,-2.0) {\includegraphics[width=11mm]{images/teaser/aug4}}; % bottom left
\node [anchor=south west, inner sep=0] at (4.9,-2.0) {\includegraphics[width=11mm]{images/teaser/aug3}}; % bottom right
\draw [white, dashed, line width=0.75, opacity=0.75] (3.8,-1.39) -- (6.02,-1.39) {};
\draw [white, dashed, line width=0.75, opacity=0.75] (4.9,-2.0) -- (4.9,-0.78) {};
\draw [black, line width=0.75] (3.8,-2.0) rectangle (6.0,-0.78) {};
\node at (4.9,-2.3) {\small $\hat{\textbf{X}}_T$};

%
% Arrows
%

\fill [fill=blue!75, opacity=0.75] (2.3,1.22) -- (3.7,0.61) -- (2.3,0.61);
\fill [fill=blue!75, opacity=0.75] (2.3,0.61) -- (3.7,0.61) -- (2.3,-2.0);
\node at (2.9,0.56) {\small \color{white}{ ConfMix}};

\fill [fill=red!75, opacity=0.75] (2.5,-2.0) -- (3.7,-1.39) -- (2.5,-1.39);
\fill [fill=red!75, opacity=0.75] (2.5,-1.39) -- (3.7,-1.39) -- (2.5,-0.78);
\node at (2.97,-1.362) {\small \color{white}{ \ourmethod}};

\end{tikzpicture}
}

\end{figure}


==> tables/abl_augm.tex <==
\begin{table}[hbt!]
\fontsize{5pt}{5pt}\selectfont
\centering
\tabcolsep 3pt
\caption{
Effect of augmentation types on the performance (mAP) for different adaptation scenarios. C: Cityscapes. F:FoggyCityscapes. S:Sim10K. K:KITTI.
\fabiocomment{add the keys to interpret/define the acronyms \hl{done}}
}
\smallskip
\begin{tabular}{lcccccc}
\toprule
Transformation & C$\to$F & K$\to$C & S$\to$C & Avg. \\
\toprule
None & 33.5 & 52.8 & 57.4 & 47.9 \\
\midrule
Horizontal Flip & 38.0 & 52.9 & 59.7 & 50.2 \\
Random Crop & 34.3 & 52.2 & 59.4 & 48.7 \\
Blur & 35.9 & 53.2 & 58.4 & 49.2 \\
Color Jittering & 34.6 & 52.5 & 58.2 & 48.5 \\
Downscale & 35.3 & 54.1 & 59.8 & 49.8 \\
Brightness Contrast & 33.9 & 52.6 & 57.5 & 48.0 \\
\midrule
HF+B & 38.9 & 53.9 & 59.3 & 50.7 \\
HF+D & 35.4 & 53.3 & 56.7 & 48.5 \\
D+B & 36.8 & 53.5 & 59.9 & 50.0 \\
\midrule
HF+D+B & 37.8 & 54.0 & 57.1 & 49.6 \\
\midrule
All & \textbf{39.4} & \textbf{54.2} & \textbf{60.6} & \textbf{51.4} \\
\bottomrule
\end{tabular}
\label{tab:abl_augm}
\end{table}


==> tables/abl_layout.tex <==
\begin{table}[hbt!]
\fontsize{5pt}{5pt}\selectfont
\centering
\caption{
Effect of grid layout on the performance (mAP) for different adaptation scenarios.  C: Cityscapes. F:FoggyCityscapes. S:Sim10K. K:KITTI. 
}
\smallskip
\begin{tabular}{ccccc}
\toprule
Layout & C$\to$F & K$\to$C & S$\to$C & Avg. \\
\toprule
3$\times$3 & 37.8 & 51.2 & 57.7 & 48.9 \\
2$\times$3 & 38.5 & 51.7 & 58.7 & 49.6 \\
3$\times$2 & 38.6 & 53.6 & 59.9 & 50.7 \\
2$\times$2 & \textbf{39.4} & \textbf{54.2} & \textbf{60.6} & \textbf{51.4} \\
\bottomrule
\end{tabular}
\label{tab:layout}
\end{table}


==> tables/abl_perc.tex <==
\begin{table}[hbt!]
\caption{
Effect of the ratio of pseudo-detections on the mAP for different adaptation scenarios. pseudo-detections ratio
}
\begin{center}
\begin{tabular}{c|cccccc}
\hline
Ratio & C$\to$F & K$\to$C & S$\to$C & Avg \\
\hline
 33\% & \hl{tba} & \hl{tba} & \hl{tba} & \hl{tba} \\
 66\% & \hl{tba} & \hl{tba} & \hl{tba} & \hl{tba} \\
100\% & 39.41 & 54.24 & 60.63 & 51.43 \\
\hline
\end{tabular}
\end{center}
\label{tab:abl_perc}
\end{table}

==> tables/abl_regions.tex <==
\begin{table}[hbt!]
\fontsize{5pt}{5pt}\selectfont
\centering
\tabcolsep 3pt
\caption{
Effect of the number of augmented regions in the 2 $\times$ 2 layout on the performance (mAP) for different adaptation scenarios. C: Cityscapes. F:FoggyCityscapes. S:Sim10K. K:KITTI. 
}
\medskip
\begin{tabular}{ccccc}
\toprule
Regions & C$\to$F & K$\to$C & S$\to$C & Avg. \\
\toprule
1 & 35.4 & 51.5 & 56.6 & 47.8 \\
2 & 38.3 & 52.2 & 58.5 & 49.7 \\
3 & 39.1 & 53.1 & 60.2 & 50.8 \\
4 & \textbf{39.4} & \textbf{54.2} & \textbf{60.6} & \textbf{51.4} \\
\bottomrule
\end{tabular}
\label{tab:regions}
\end{table}

